PCEDNet : A Lightweight Neural Network for Fast and Interactive Edge Detection in 3D Point Clouds

In recent years, Convolutional Neural Networks (CNN) have proven to be efficient analysis tools for processing point clouds, e.g., for reconstruction, segmentation and classification. In this paper, we focus on the classification of edges in point clouds, where both edges and their surrounding are described. We propose a new parameterization adding to each point a set of differential information on its surrounding shape reconstructed at different scales. These parameters, stored in a Scale-Space Matrix (SSM), provide a well suited information from which an adequate neural network can learn the description of edges and use it to efficiently detect them in acquired point clouds. After successfully applying a multi-scale CNN on SSMs for the efficient classification of edges and their neighborhood, we propose a new lightweight neural network architecture outperforming the CNN in learning time, processing time and classification capabilities. Our architecture is compact, requires small learning sets, is very fast to train and classifies millions of points in seconds.

==> tex/03_overview.tex <==

\section{Overview}


\subsection{Architectures}
\label{sec:networkarchitectures}

%%Deciding which architecture to use is not an easy task, considering the lack of examples. The architecture design followed a trial-and-error process to achieve our final architecture proposal.
Our architecture proposal is the result of a very large number of trial-and-errors, from larger and deeper networks, including convolution or not, to even simpler designs. 
% so we went with different architectures and by the process of testing and exclusion, we arrived at a number of different candidates for a good architecture for this kind of process. % T: replace this sentence with sth like: The architecture design followed a trial-and-error process to achieve our final architecture proposal.

We classify and set different architectures based on their efficiency (Speed / Accuracy), speed is required considering that the network would be used to classify large point clouds (millions to billions of points).
%and since % T: since?increasing the speed (reduction in network size) would end up reducing the accuracy of the network, it was clear that the perfect network resides in balance between these two factors. % T: this last part of the sentence is not necessary to me, from: and since ...



